DLBricks: Composable Benchmark Generation to Reduce Deep Learning Benchmarking Effort on CPUs (Extended)

The past few years have seen a surge of applying Deep Learning (DL) models for a wide array of tasks such as image classification, object detection, machine translation, etc. While DL models provide an opportunity to solve otherwise intractable tasks, their adoption relies on them being optimized to meet latency and resource requirements. Benchmarking is a key step in this process but has been hampered in part due to the lack of representative and up-to-date benchmarking suites. This is exacerbated by the fast-evolving pace of DL models. This paper proposes DLBricks, a composable benchmark generation design that reduces the effort of developing, maintaining, and running DL benchmarks on CPUs. DLBricks decomposes DL models into a set of unique runnable networks and constructs the original model's performance using the performance of the generated benchmarks. DLBricks leverages two key observations: DL layers are the performance building blocks of DL models and layers are extensively repeated within and across DL models. Since benchmarks are generated automatically and the benchmarking time is minimized, DLBricks can keep up-to-date with the latest proposed models, relieving the pressure of selecting representative DL models. Moreover, DLBricks allows users to represent proprietary models within benchmark suites. We evaluate DLBricks using $50$ MXNet models spanning $5$ DL tasks on $4$ representative CPU systems. We show that DLBricks provides an accurate performance estimate for the DL models and reduces the benchmarking time across systems (e.g. within $95\%$ accuracy and up to $4.4\times$ benchmarking time speedup on Amazon EC2 c5.xlarge).

==> Makefile <==
LATEX=pdflatex
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf
CONTINUOUS=-pvc

SOURCES=main.tex Makefile $(shell find sections/* -type f)
FIGURES := $(shell find figs/* -type f)

all: force

.refresh:
	touch .refresh

main.pdf: main.tex .refresh $(SOURCES) $(FIGURES)
    $(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
        -pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" main

force:
	touch .refresh
	rm -fr main.pdf
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
		-pdflatex="$(LATEX) $(LATEXOPT) %O %S" main

clean:
	$(LATEXMK) -C main
	rm -f main.pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" main

debug:
	$(LATEX) $(LATEXOPT) main

.PHONY: clean force once all

==> latex_tools/yaml.tex <==




\definecolor{yamlred}{rgb}{0.843137,0.188235,0.152941}
\definecolor{yamlblue}{rgb}{0.27451,0.32549,0.384314}
\definecolor{yamlkey}{rgb}{0.980392,0.501961,0.447059}

\newcommand\YAMLfontsize{\fontsize{6}{6}}
\newcommand\YAMLfontstyle{\ttfamily}
\newcommand\YAMLcolonstyle{\color{black}\mdseries\YAMLfontsize\YAMLfontstyle}
\newcommand\YAMLkeystyle{\bfseries\color{yamlblue}\YAMLfontsize\YAMLfontstyle}
\newcommand\YAMLvaluestyle{\color{black}\mdseries\YAMLfontsize\YAMLfontstyle}



% here is a macro expanding to the name of the language
% (handy if you decide to change it further down the road)

\definecolor{yamlgray}{rgb}{0.5,0.5,0.5}
\lstdefinelanguage{yaml}
{
  keywords={true,false,null,y,n},
  keywordstyle=\YAMLvaluestyle,
  basicstyle=\YAMLfontsize\YAMLkeystyle,                                 % assuming a key comes first
  sensitive=false,
  comment=[l]{\#},
  morecomment=[s]{/*}{*/},
  commentstyle=\YAMLcolonstyle\color{yamlred}\YAMLfontstyle\YAMLfontsize\YAMLfontstyle,
  stringstyle=\YAMLvaluestyle\YAMLfontstyle\YAMLfontsize\YAMLfontstyle,
  moredelim=[l][\color{orange}]{\&},
  moredelim=[l][\color{yamlred}]{*},
  moredelim=**[il][\YAMLcolonstyle{:}\YAMLvaluestyle]{:},   % switch to value style at :
  morestring=[b]',
  morestring=[b]",
  literate =    {---}{{\ProcessThreeDashes}}3
                {>}{{\textcolor{yamlred}\textbar}}1     
                {|}{{\textcolor{yamlred}\textbar}}1 
                {\ -\ }{{\mdseries\ -\ }}3,       
    % frame=single,
    frame=top,
    frame=bottom,
    numbers=left,
    framerule=1pt,
    rulesep=1pt,
	breaklines=true,
    mathescape=true,
    xleftmargin=0em,
    framexleftmargin=0em,
    xrightmargin=0pt,
    stepnumber=1,
    escapechar=|,
    captionpos=t,
    escapeinside={(*}{*)},
    numberstyle=\ttfamily\tiny\color{yamlgray},
}

% switch to key style at EOL
% \lst@AddToHook{EveryLine}{\ifx\lst@language yaml\YAMLkeystyle\fi}
\makeatother

\newcommand\ProcessThreeDashes{\llap{\color{cyan}\mdseries-{-}-}}


==> sections/4.1-sharing.tex <==
\subsection{Subgraph Sharing among DL models}\label{sec:sharing}

Models within the same category share subgraphs that are only differ in input and output shapes.

Figure~\ref{fig:sharing_wo_relax} shows the layer sharing among models within each category in https://reference.wolfram.com/language/tutorial/NeuralNetworksOverview.html.

Figure~\ref{fig:sharing_w_relax} shows the layer sharing with relaxation (using \circledwhite{2}) among models within each category.

Figure~\ref{fig:sharing_w_relax_n} shows the subgraph (numlayers to be 2, 3, ..., 10) sharing with relaxation  (using \circledwhite{2}) among models within each category.

\begin{figure}[ht]
	\centering
	\includegraphics[draft,width=0.48\textwidth]{figures/sharing_wo_relax.pdf}
	\caption{
	}
	\label{fig:sharing_wo_relax}
	\vspace{-10pt}
\end{figure}


\begin{figure}[ht]
	\centering
	\includegraphics[draft,width=0.48\textwidth]{figures/sharing_w_relax.pdf}
	\caption{
	}
	\label{fig:sharing_w_relax}
	\vspace{-10pt}
\end{figure}

\begin{figure}[ht]
	\centering
	\includegraphics[draft,width=0.48\textwidth]{figures/sharing_w_relax_n.pdf}
	\caption{
	}
	\label{fig:sharing_w_relax_n}
	\vspace{-10pt}
\end{figure}

==> sections/4.1.2-relaxation.tex <==

\subsubsection{Relaxation Rules}\label{sec:relax}

After decomposing models into layer sequences, the benchmark generator takes the union of all the sequences and produces a set of unique sequences as the benchmarks.
To minimize the number of generated benchmarks and reduce benchmarking time and effort, \proj{} defines "relaxation rules" for different layer types that correlate a layer's performance to another layer.
If two layers' performance can be correlated, only one of them needs to be in the generated benchmarks and the one that requires less time is chosen.


\input{sections/fig_layer_distribution_per_task.tex}


\begin{figure}[ht]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/layer_distribution_per_task/all_tasks.pdf}
	\caption{
		Layer distribution of models within each category in Table~\ref{tab:models_full}.
	}
	\label{fig:all_tasks}
	\vspace{-10pt}
\end{figure}

Figure~\ref{fig:all_tasks} shows the layer distribution of all the model and Figure~\ref{fig:layer_distribution_per_task} shows the layer distribution of the models within each task.
We look at the top $15$ layer types of the models to find the relaxation rules for them.
We examine the layer parameters, calculate the theoretical flops~\cite{}, and measure the runtime for the layers.
Figure~\ref{fig:relax} shows for each common layer types and the layers the layer parameters (or flops) vs layer latency.

We find that convolution layers are compute bound and are optimized on CPUs in a non-trivial way, thus no parameter-related correlation can be found between two convolution layers.
For other memory-bound layers such as batchnormalization and element-wise layers, two layers can be correlated with the theoretical flops (calculated from layer parameters) on CPUs.
In summary, we come up with the relaxation rules in Table~\ref{tab:relaxation_rules} for different layer types.




Assume $layer_1$ is of shape $[x_1,y_1,z_1]$, $layer_2$ is of shape $x_2, y_2, z_2$, We define the relaxation rules for different layer types as follows.

\begin{itemize}
	\item Convolution: $layer_1$ and $layer_2$ have the same kernel, stride, dilation, and output shape, then $\frac{T_{layer_1}}{T_{layer_2}} =\frac{flops_{layer_1}}{flops_{layer_2}} = \frac{Input Chanel_{layer_1}}{Input Chanel_{layer_2}}$.
	\item BatchNorm: $x_1*y_1*z_1 == x_2*y_2*z_2 => T_{layer_1} = T_{layer_2}$.
	\item Relu: $[x, y, z]  => x*y*z$.
	\item Element-wise: $layer_1$ and $layer_2$ have the same element-wise function, such as ramp, then $\frac{T_{layer_1}}{T_{layer_2}} = \frac{flops_{layer_1}}{flops_{layer_2}}$.
	\item Pooling: $[x, y, z]  => x*y*z$.
	\item Total: $layer_1$ and $layer_2$ have the same input shapes and output shape, then $T_{layer_1} = T_{layer_2}$.
	\item Other layer types: all the parameters of $layer_1$ and $layer_2$ are the same, then $T_{layer_1} = T_{layer_2}$.
\end{itemize}






\begin{figure}
	\centering
	\includegraphics[clip,width=0.48\textwidth]{figures/across_model_flop_sharing.pdf}
	\caption{The sharing grid of the models in Table~\ref{tab:models}. Red indicates layer sharing exists between the two models with the defined relaxation rules, and black means there is no sharing.}
	\label{fig:sharing_w_relax}
\end{figure}

\begin{figure}[ht]
	\centering
	\includegraphics[draft,width=0.48\textwidth]{figures/across_model_sharing_relaxed.pdf}
	\caption{
	}
	\label{fig:across_model_sharing_relaxed}
	\vspace{-10pt}
\end{figure}

Figure~\ref{fig:across_model_sharing_relaxed} shows the layer sharing between the models in Table~\ref{tab:models_full} after applying the relaxation rules defined above.


==> sections/5.3-other_modalities.tex <==

\subsection{Applicability to Other Models}

Describe RNN, LSTM, etc. properties.
Dynamic graphs can be traced to create a static graph.

To validate the premise of our methodology, we evaluate our claims on other modalities.
Table~\ref{tbl:eval-other} shows that other there is extensive sharing of layers within a model.
Our code generation implementation currently only supports ONNX OpSet $7$, and thus does not currently support the generation of benchmarks for these models.

\begin{table}
	\centering
	\resizebox{0.48\textwidth}{!}{%

		\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l c r r} \toprule
			\centering%
			\textbf{\thead{Model}} &  \textbf{\thead{Task}} & \textbf{\thead{\#Layer}} & \textbf{\thead{\#Unique}}  \\ \midrule
			Bert~\cite{devlin2018bert} & \textbf{LM} & 862 & 19 \\
			Deep Speech 2~\cite{amodei2016deep} & \textbf{SR} & 152 & 33 \\
			Elmo~\cite{peters2018deep} & \textbf{FE} & 111 & 41 \\  %
			GPT~\cite{radford2018improving} & \textbf{LM} & 857 & 15 \\
			GPT-2~\cite{radford2019language} & \textbf{LM} & 832 & 14 \\ %
			\bottomrule
		\end{tabular*}%
	}
	\caption{
		Number of total layers and unique layers within networks that represent the Language Modeling (\textbf{LM}),  Speech Recognition (\textbf{SR}), and Feature Extraction (\textbf{FE}) modalities.
	}
	\label{tab:eval-other}
	\setlength{\belowcaptionskip}{-13pt}
	\vspace{-10pt}
\end{table}

If we concentrate on transformer networks used for language modeling \textbf{LM}.
The transformer networks represent words as a sequence of vectors with Bert~\cite{devlin2018bert}, GPT~\cite{radford2018improving}, and GPT-2~\cite{radford2019language} being state-of-the-art.
Looking within a transformer model, for example, the GPT model has $857$ layers of which only $15$ are unique.
In total, Bert, GTP, and GTP-2 have $2551$ of which $48$ are unique --- or $1.9\%$ of the layers are unique.
There are variants of the GPT models, solving slightly different tasks within the the text-processing domain.
Looking at these (omitted for brevity) results in ample intra-model layer sharing.




==> sections/fig_layer_distribution_per_task.tex <==

\begin{figure*}
	\centering
	\begin{subfigure}[b]{0.30\textwidth}
		\includegraphics[width=\textwidth]{figures/layer_distribution_per_task/Audio_Analysis.pdf}
		\caption{Audio Analysis}
		\label{fig:layer_distribution_per_task:aa}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.30\textwidth}
		\includegraphics[width=\textwidth]{figures/layer_distribution_per_task/Classification.pdf}
		\caption{Image Classification}
		\label{fig:layer_distribution_per_task:ic}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.30\textwidth}
		\includegraphics[width=\textwidth]{figures/layer_distribution_per_task/Feature_Extraction.pdf}
		\caption{Feature Extraction}
		\label{fig:layer_distribution_per_task:fee}
	\end{subfigure}
	\\
	\begin{subfigure}[b]{0.30\textwidth}
		\includegraphics[width=\textwidth]{figures/layer_distribution_per_task/Image_Processing.pdf}
		\caption{Image Processing}
		\label{fig:layer_distribution_per_task:ip}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.30\textwidth}
		\includegraphics[width=\textwidth]{figures/layer_distribution_per_task/Language_Modeling.pdf}
		\caption{Language Modeling}
		\label{fig:layer_distribution_per_task:lm}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.30\textwidth}
		\includegraphics[width=\textwidth]{figures/layer_distribution_per_task/Object_Detection.pdf}
		\caption{Object Detection}
		\label{fig:layer_distribution_per_task:od}
	\end{subfigure}
	\\
	\begin{subfigure}[b]{0.30\textwidth}
		\includegraphics[width=\textwidth]{figures/layer_distribution_per_task/Regression.pdf}
		\caption{Regression}
		\label{fig:layer_distribution_per_task:reg}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.30\textwidth}
		\includegraphics[width=\textwidth]{figures/layer_distribution_per_task/Semantic_Segmentation.pdf}
		\caption{Semantic Segmentation}
		\label{fig:layer_distribution_per_task:ss}
	\end{subfigure}
	~
	\begin{subfigure}[b]{0.30\textwidth}
		\includegraphics[width=\textwidth]{figures/layer_distribution_per_task/Speech_Recognition.pdf}
		\caption{Speech Recognition}
		\label{fig:layer_distribution_per_task:sr}
	\end{subfigure}
	\caption{XXX}
	\label{fig:layer_distribution_per_task}
\end{figure*}
